Extending the View Composition Algebra to Hierarchical Data

Comparison is a core task in visual analysis. Although there are numerous guidelines to help users design effective visualizations to aid known comparison tasks, there are few formalisms that define the semantics of comparison operations in a way that can serve as the basis for a grammar of comparison interactions. Recent work proposed a formalism called View Composition Algebra (VCA) that enables ad hoc comparisons between any combination of marks, trends, or charts in a visualization interface. However, VCA limits comparisons to visual representations of data that have an identical schema, or where the schemas form a strict subset relationship (e.g., comparing price per state with price, but not with price per county). In contrast, the majority of real-world data - temporal, geographical, organizational - are hierarchical. To bridge this gap, this paper presents an extension to VCA (called VCAH) that enables ad hoc comparisons between visualizations of hierarchical data. VCAH leverages known hierarchical relationships to enable ad hoc comparison of data at different hierarchical granularities. We illustrate applications to hierarchical and Tableau visualizations.

==> content/algebra.tex <==
\section{\sys for Database-oriented Visual Analytics}
\label{s:algebra}

This section defines the semantics of \sys for visual analytics. We first define view tables as SQL group-by aggregation queries, and then define the operator semantics---specifically, the data transforms and visual mappings of the output view given the operator inputs.   Please refer to next section  for diagrams and screenshots of the interaction designs to express these operators.

\subsection{View Definition}

As described in \Cref{ss:vcaoverview} we model a view as $V_i = R_i(T_i)$.
In visual analytic systems, $T_i$ is typically the output of a transformation query $Q_i(D)$ over an input database table $D$.  Our algebra will be defined over such queries.  Let $D(a_1,\ldots,a_n)$ contain $n$ attributes and $A_D = [a_1,\ldots,a_n, a_y]$ denote its schema, where $a_y$ is the measure, and the rest are dimensions.
$Q_i$ is responsible for all data processing and transformation (e.g., grouping, filtering, joining with other tables), so that rendering simply maps each result row to a mark rendered in the view.    The separation of data transformation and
presentation allows each to be defined and changed independently.
%For convenience, we will use $Q_i$ and $Q_i(D)$ interchangeably.


\subsubsection{Query Transformation}\label{ss:algebra-query}
\input{content/relalgtable}

Most visual analytic systems~\cite{Stolte2000PolarisAS,dice2014,Gray2004DataCA,Chaudhuri1997AnOO,Pahins2017HashedcubesSL} are based on {\it group-by aggregation queries} that filter the input
table using a predicate $p$, group records by a set of attributes $A_{gb}$, and compute an aggregated statistic $f_i(a_y)$:
%
  \begin{lstlisting}[
    caption={},
    captionpos=b,
    basicstyle=\small\ttfamily,
    frame=,
    mathescape=true,
    escapeinside={@}{!} ]
  $Q_i$ = SELECT @$A_{gb}$!, @$f(a_y)\to y$!  FROM D [WHERE @$p$!] GROUP BY @$A_{gb}$!
  \end{lstlisting}
%
  \noindent For example, VizQL is a layout algebra for creating faceted, layered charts from relational databases whose statements are translated into group-by aggregation queries~\cite{stolte03thesis}.  \Cref{a:vizql} describes how VizQL statements are expressible as operands in \sys.  

SQL is verbose and difficult to symbolically manipulate, so we will use the equivalent relational algebra statements (\Cref{t:relalg}):

  $$Q_i = \gamma_{A_{gb}, f(a_y)\to y}(\sigma_{p}(D))$$

\noindent $\sigma$ keeps rows that satisfy predicate $p$, $\gamma$ groups rows by a subset of the dimensions $A_{gb}$ and computes  $f(a_y)$ for each group.  

\begin{figure*}
   \centering
   \includegraphics[width=\linewidth]{algebra_ops}
   \vspace{-2em}
   \caption{Examples of View Composition Algebra operations over views of flight delay statistics.  
     The algebra enables comparison and composition of visualization views.  
     (a) difference between SFO and OAK delay statistics by date,
     (b) the sum of delays by date,
     (c) union composition of SFO and OAK delays,
     (d) difference between 1D SFO delays and a 0D delay constant,
     (e) difference between a 2D heat map of delays per city, date, and a 1D view of El Paso delays,
     (f) fit linear models to extrapolate AM and PM delay trends. 
   }
 	\label{f:algebra_ops}
\end{figure*}



\subsubsection{Visual Mapping}

Each output record of $Q_i$ is mapped to one mark.  
Given the view's mark type $K$, $R_i$ maps 
attributes in the query result to visual attributes  (e.g., x, y, color) valid for the mark type $K$. 
Let $A_{Q_i}$ be the attributes in $Q_i$, and $A_K$ be the set of visual attributes for $K$.  $R_i$ is defined as:
$$R_i = \{K\to mark\} \cup \{ a_q\to a_v | a_q\in A_{Q_i} \land a_v\in A_K \}$$
Each visual attribute can be referenced at most once, and not all query attributes need to be mapped.  Let $A_{R_i}$ denote the visual attributes that have been mapped in $R_i$.

Our algebra incorporates Gleicher et al.'s three design strategies for visual comparison (juxtaposition, superposition, and explicit encoding)~\cite{gleichercompare} depending on the operator.  The user can then use existing mechanisms to reconfigure the output view's visual mappings or recommend alternative mappings~\cite{Mackinlay2007ShowMA,Moritz2019FormalizingVD,Lin2020DzibanBA}, since they are well-supported in visual analysis systems.

%\begin{figure}[b]
%  \centering
%  \includegraphics[width=.75\columnwidth]{figs/viewdef}
%  \vspace{-1em}
%  \caption{A view $V$ in \sys is defined as a data transformation and processing query $Q$ 
%  whose result is directly mapped to marks by $R$.}
%  \label{f:viewdef}
%\end{figure}



%\begin{example}\label{ex:1}
%  The table \texttt{flight(date, hour, src, dst, delay)} tracks airplane arrival delay statistics.
%  \Cref{f:viewdef} filters flights from California (\texttt{src=CA}), 
%  computes the attribute \texttt{ampm} from \texttt{hour},
%  groups the resulting records by $A_{gb} = [date, ampm]$, 
%  and computes the average delay for each group.  $Q$ is expressed as:
%  \begin{align*}
%  \gamma_{date, ampm, avg(delay)\to delay}\left( \pi_{*, hour<12\to ampm}\left(
%    \sigma_{src='CA'}\left(D  \right)   \right) \right) 
%  \end{align*}
%  \noindent To render the scatter plot, 
%  $R$ maps each row to a point, 
%  date to the x axis, delay to the y axis, and ampm to color.
%  $$\{`point'\to mark, date\to x, delay\to y, ampm\to color\}$$.
%\end{example}




\subsection{Binary View Composition}


A binary operator takes views $V_1$ and $V_2$ as input and returns a new view $V^* = R^*\left( Q^* \right) $.  
The statistical operator $\odot_\phi$ derives new statistics from the input views' measures, and
the union operator $\cup_\phi$ merges their data into the same view, and the operator parameter $\phi$ is described below.
\Cref{f:algebra_ops}(a-c) illustrate these binary operators.
Recall that the input views are compatible if the measures are compatible and the set of dimensions are the same.  We will relax the latter requirement in \Cref{sss:schema} to support compositions such as \Cref{f:algebra_ops}(d,e).

\subsubsection{Statistical Composition $\odot$}
\label{ss:algebra_stat}

$V^*=V_1\odot_{op} V_2$ joins rows from $Q_1$ and $Q_2$ and computes a new measure $Q_1.y\ op\ Q_2.y$ from the two views' measures:
\begin{align*}
  Q^* &= \pi_{A_{gb}, Q_1.y\ op\ Q_2.y\to y }\left(Q_1 \fullouterjoin_{A_{gb}} Q_2  \right) \\
  R^* &= R_1
\end{align*}
%
$Q^*$ first computes the outer join between $Q_1$ and $Q_2$ by matching records from each query 
whose grouping attributes  $A_{gb}$ have the same values.  
An outer join ensures that rows in either table have at least one output row even if there is no match.
Since the input queries, by definition, were grouped on $A_{gb}$, we are guaranteed exactly one output row for each group in $Q_1$ and $Q_2$.  Finally, $\pi$ copies the join attributes, computes $Q_1.y\ op\ Q_2.y$, and renames it as $y$.


$op$ is defined as ``$-$'' by default, however any binary arithmetic function is allowed.
As shorthand, $\oplus$ and $\ominus$ denote $\odot_+$ and $\odot_-$, respectively.
$\odot_{op}$ is symmetric iff $y_1\ op\ y_2 = y_2\ op\ y_1$.

There is one special case where the right operand $V_2$ is handled differently 
than described above.  If a grouping attribute $a\in A_{gb}$ 
only contains a single unique value in $Q_2$'s output,
we remove $a$ from $Q_2$'s grouping attributes.
This is so dimension attributes that do not encode any data variation 
do not affect the semantics of the operator.  
This case is then handled as nonexact schema composition (\Cref{sss:schema}).


\begin{example}
\Cref{f:algebra_ops}(a) subtracts \texttt{OAK} daily delays from \texttt{SFO} daily delays.  
Since the queries for both views group by \texttt{date, src}, a naive composition
will join the two datasets on $A_{gb}=[date,src]$ and none of the rows will match.
In contrast, dropping \texttt{src} from the join condition is needed compare each \texttt{SFO} day to the correspoding day in \texttt{OAK}.
\end{example}

\subsubsection{Union Composition $\cup$}

Union $V^* = V_1\cup_{qid,a}V_2$ composes the marks from both views into the same output view:
\begin{align*}
  Q^* & = \pi_{*, \hl{qid}}(Q_1) \cup \pi_{*, \hl{qid}}(Q_2) \\
  R^* &= \{qid\to\hl{$a$}\} \cup R_1 \hspace{2em} s.t. \ a \in A_K - A_{R_1}
\end{align*}
%
Each query $Q_i$ is augmented to track a unique identifier $qid$, so that rows from each query can be distinguished in $Q^*$.  $R^*$ additionally maps $qid$ to a visual attribute $a$ that is not already mapped in $R_1$.

By default, $qid$ is defined based on an internal identifier for the input view. However, it can be any value that uniquely identifies the view.  For instance, if the input views are part of a faceted visualization, then $qid$ may be each view's facet title.   By default, $a$ uses existing perceptual effectiveness orderings~\cite{cleveland1984graphical,Stolte2000PolarisAS} to choose the most effective ordinal visual attribute that is available.

Union composition will juxtapose (as in \Cref{f:algebra_ops}(c)) or superimpose (as in \Cref{f:teaser}(b)) the input marks based on their mark type.  If the mark fills the area between the measure value and 0 (e.g., bar charts, area charts), then the marks in the output view are juxtaposed to avoid overlapping them.  In contrast, line and scatterplot marks are simply superimposed atop each other.

\subsection{Statistical Composition with Nonexact Schemas}
\label{sss:schema}

\Cref{f:algebra_ops}(d,e) are examples where the two views do not have identical query schemas.
They measure the difference between a bar chart and a constant value, or between a heat map and a bar chart.   
We now relax the safety rules for statistical composition $\odot_{op}$ to cases where the set of grouping attributes $A_{gb}^1$ in $Q_1$ 
is a strict super set of $A_{gb}^2$ in $Q_2$. 
\begin{align*}
  Q^* &= \pi_{A_{gb}^1, Q_1.y\ op\ Q_2.y\to y }(Q_1 \leftouterjoin_{A_{gb}^2} Q_2)\\
  R^* &= R_1
\end{align*}
%
$Q^*$ is defined over the {\it left} outer join of 
$Q_1$ and $Q_2$.  This join ensures that rows in $Q_1$ are preserved in the join
result, but rows in $Q_2$ that do not have a join match are not in the output.
We chose this because composition of views with different schemas is not 
symmetric---$V_1$ is transformed by matching data in $V_2$, but not vice versa.

How $A^2_{gb}$ is defined for $Q_2$ affects the semantics of the operator.  If $Q_2$ does not have any grouping attributes---it only contains a metric attribute---then every mark in $V_1$ will be composed with every metric value in $V_2$.  However, if $Q_2$ contains a \texttt{date} dimension, then each mark in $V_1$ will only be composed with the metric values in $V_2$ that have the same \texttt{date}.
Finally, note that the join condition is with respect to the smaller set of 
grouping attributes in $Q_2$,
whereas the attributes preserved in the query output are from $Q_1$.


\begin{example}
\Cref{f:algebra_ops}(d) composes a 1D view of SFO delays ($V_1$) with a 0D view ($V_2$) 
consisting of a single delay constant.
Their grouping attributes correspond to $A_{gb}^1=[date]$ and $A_{gb}^2=\emptyset$.
$V_1\ominus V_2$ subtracts the constant from each row in $Q_1$.
\end{example}

\begin{example}
\Cref{f:algebra_ops}(e) composes a 2D heat map of delays by city$\times$date ($V_1$)
with a 1D bar chart of El Paso delays by date ($V_2$).  Their grouping attributes are $A_{gb}^1=[date, city]$ and $A_{gb}^2=[date]$, and the resulting view removes El Paso's 
delays from each city's delays.
\end{example}


\subsection{View Decomposition}\label{ss:decompose}

It is often useful to decompose components of a view (values, marks, groups) into one or more stand-alone views that contain a subset of the input view's rows and attributes.  The new views can then be used as operands for further composition, or manipulated for further analysis.  To this end, we define 2 decomposition operators based on interactions often used during view manipulation and coordination.   

The {\it extract} operator $\downarrow(V, p) = R(\sigma_p(Q))$ creates a single new view based on a subset of rows in $V$ that match predicate $p$.  If $p$ is not specified, it defaults to $true$, which is equivalent to creating a copy of $V$.  $\downarrow$ can be used to create a standalone view that renders a selected subset of marks, similar to coordinated overview-detail visualizations.   $\downarrow$ can also be used to e.g., extract marks from different views and then juxtapose them using $\cup$.  

The {\it explode} operator $\Xi_{A_e}(V)$ generates a set of views (a viewset), with one view for each group defined by the attributes $A_e$.   Explode is similar to facetting, which is traditionally used when creating new views from raw data.  In contrast, $\Xi$ is directly applied to existing views, including views derived from previous manipulations or compositions.  The query for each output view first filters by the group, and then drops the explode attributes $A_e$; the visual mapping drops any mappings from $A_e$:
\begin{align*}
  \mathbb{Q}^* &= \{\pi_{\neg A_e}(\sigma_{A_e=vals}(Q)) | vals \in \gamma_{A_e}(Q)  \}\\
  R^* &= \{a\to a_v | a\to a_v\in R \land a\not\in A_e \}\\
  \mathbb{V}^* &= \{ R^*(Q^*) | Q^* \in \mathbb{Q}^* \}\\
      \neg A_e &= A_{gb} - A_e
\end{align*}




\subsection{Composing Viewsets}\label{ss:viewsets}

We now extend composition to a {\it viewset} containing $n$ views 
$\mathbb{V} = \{V_1,\ldots,V_n\}$.  
Following our safety rules, all views in $\mathbb{V}$ have identical schemas, and
their queries  have the same grouping attributes $A_{gb}$.  

\subsubsection{Viewset Statistical Composition $\odot$}

When statistically composing a viewset $V^* = \odot_{f^*}(\mathbb{V})$, 
the purpose is to derive new statistics from the underlying data of each of the views,
rather than compare any individual pair of views in the viewset.
For this reason, we first union the {\it preaggregated} data from each query, and then
{\it reaggregate} the union.  
These semantics differ from binary statistical composition, which composes the aggregated measures from each input query.

We first rewrite each $Q_i$ as $\gamma_{A_{gb}, f(a)\to y}(q_i)$, 
where $q_i$ represents any filtering, join, and projection
operations that $Q_i$ performs prior to grouping and aggregation ($\gamma$).
This does not change the semantics of $Q_i$, but allows us to refer to $q_i$ in the definition above.
%
\begin{align*}
  Q^* &= \gamma_{A_{gb}, \hl{$f^*(a)$}\to y}\left(q_1 \cup \ldots \cup q_n  \right) \\
  R^* &= R_1
\end{align*}
%
$Q^*$ first unions all $q_i$ before grouping by $A_{gb}$ and 
computing the aggregation function \hl{$f^*\left(  \right)$}.  
We do this to ensure that aggregate statistics are always computed over the input data, 
and so users do not inadvertantly compute e.g., averages of averages, 
which can easily lead to misinterpretation. 
Common aggregations include \texttt{min}, \texttt{max}, \texttt{avg}, \texttt{std}, and \texttt{count}, however any 
numeric aggregation function (e.g., $\frac{avg(delay)}{max(delay)}$ is acceptable.
We use $f^*\left(  \right) $ to distinguish the parameter from the non-aggregation function 
$h\left(  \right)$ used in binary composition and the aggregation $f\left( \right)$ in the input
queries.

We also generalize the special case in binary statistical composition to every view in the viewset.   
If a grouping attribute $a$ has
a single unique value in {\it every} view's query result, then it is removed from 
$A_{gb}$ when computing the group by in $Q^*$.
For instance, if the user highlights a set of marks in a chart, and wants to summarize
their measures, then each mark is treated like a separate view, and their grouping attributes are
all dropped (since there is a single group in each ``view'').
If this is not done, the output in the example would be the same set of marks---effectively a noop.
We illustrate this interaction in \Cref{ss:iact_nary}.


\subsubsection{Viewset Union Composition $\cup$}

The union operator $V^*=\cup_{qid,a_t}(\mathbb{V})$ directly extends the 
binary union operator by extending and unioning all queries in the viewset.  
Similarly, \hl{$qid$} maps to an available visual attribute $a$.
%
\begin{align*}
  Q'_i &= \pi_{Q_i.*, \hl{qid}}(Q_i(D))\hspace{2em}\forall i\in[1,n]\\
  Q^* & = Q'_1 \cup \ldots \cup Q'_n \\
  R^* &= \{qid\to\hl{$a$}\} \cup R_1\hspace{2em} s.t. \ a \in A_K - A_{R_1}
\end{align*}



\subsubsection{Viewset-View Composition}

We can now define composition of viewsets and views, whose output is a new viewset.  Below, $\circ$ denote any binary operator:
\begin{align*}
  \mathbb{V} \circ V &= \{ V_i \circ V | V_i\in\mathbb{V} \}\\
  V \circ \mathbb{V} &= \{ V \circ V_i | V_i\in\mathbb{V} \}\\
  \mathbb{V}_1 \circ \mathbb{V}_2 &= \{ V_i \circ V_j | V_i\in\mathbb{V}_1, V_j\in\mathbb{V}_2 \}
\end{align*}


\subsection{Learning and Composing Model Views}

Oftentimes two views may not neatly compose because the {\it values} of the grouping attributes do not match.  
For instance, suppose $V_1$ renders delays on even days while $V_2$ renders  delays on odd days.  
Although $V_1\ominus V_2$ is safe, the resulting view
is uninformative because there are no matching dates in the join.
%
For this reason, the unary {\it lift} operator $\uparrow_{M,A_d, A_c}(V)$ fits a model $M$ to the data in view $V$ and returns a {\it model view}:  
\begin{align*}
  Q^* &= \gamma_{\hl{$A_c$}, train_{\hl{$M$}}(\hl{$A_d$},y)}\left(Q \right) \\
  R^* &= \{a\to a_v |  a\to a_v\in R \land a\in \hl{$A_c$}\cup \hl{$A_d$} \}\hspace{2em} s.t. \ \hl{$A_d, A_c$} \subseteq A_{gb}
\end{align*}
%
In the above, $Q^*$ groups the output of $Q$ by $A_c$, and for each group, trains a model $M$ that uses $A_d$ as features to predict the measure $y$.  In effect, the operator trains the model $M(A_d, y | A_c)$.
$R^*$ only keeps mappings in $R$ related to the features $A_d$ or conditioned attributes $A_c$.
We require that $A_d$ and $A_c$ are part of $V$'s grouping attributes, and $A_d$ contains only quantitative attributes that can be used as numeric features in the model.  


\begin{example}
  In \Cref{f:algebra_ops}(f), $\uparrow_{linear,[date],[ampm]}(V)$ fits two linear regression models, one for AM and one for PM.  Each model uses \texttt{date} and an intercept term to predict the average delay.  
\end{example}

Models are a compact representation of an infinite-sized relation, however
 charts render finite sets of rows.
In order to render a model view, we sample the domain of $A_d$ and predict
the $y$ value for each sample in each group as defined by $A_c$.  
The results are used as the ``query result'' and rendered as normal.
As a heuristic, we sample $20$ equi-distant values from the domain of each attribute in $A_d$; if there are many attributes in $A_d$, we scale down the samples per attribute so the total number of samples does not exceed $1000$.

\subsubsection{Composing a View and Model View}

A major use case for model views is to aid comparisons
between views that would otherwise not share join values.  
We define the composition  $V_1\circ V_M$ 
of a view $V_1$ and model view $V_M$ as follows, where $\circ$ is any binary composition operator and the usual safety rules apply:
\begin{align*}
  Q_M' &=  \pi_{A_{gb}^1, M(Q_1.A_d)\to y}\left( Q_1 \bowtie_{A_c} Q_M \right) \\
  V_M' &= R_M(Q_M')\\
  V^* &= V_1 \circ V_M'
\end{align*}
%
At a high level, we use the models in $V_M$ to predict the $y$ value for each
row in $Q_1$.  To do so, we need to match the appropriate model $M$ for each $Q_1$ row.  We do this using an inner join on $A_c$, which emits a join result only if there is a match.    This is to avoid the case when a model has not been trained for the specific $A_c$ values for a row in $Q_1$; we emit a warning with the number of such rows.   Each join result projects the grouping attributes $A_{gb}^1$ from $Q_1$ along with the predicted $y$ value.     If $\circ$ is symmetric, then $V_M\circ V_1 = V_1\circ V_M$.

\subsubsection{Composing Two Model Views}

In order to compose two model views, we follow the same procedure as rendering a model view.  We sample from $A_d$, and use the samples to generate predictions from both model views.  The results are treated as query results and the normal composition operator is applied.



\subsection{Properties of the Algebra}

The operators are closed---operator outputs can be inputs to other operators---except in one case.
The nary statistical composition operator assumes that the input views' queries in canonical form  $\gamma_{A, f()}(q)$, where $q$ does not contain any aggregation operators.  All operators return views with canonical queries, except for binary statistical composition $\ominus(V_1, V_2)$, whose output query structure is $\pi(Q_1\fullouterjoin Q_2)$.   In this case, aggregation happens before the join ($\fullouterjoin$) and projection ($\pi$), and in general cannot be rewritten into canonical form.

\input{content/visql.tex}


==> content/overview.tex <==
\section{Overview}  
\label{s:overview}

This section provides an overview of the view composition algebra (\sys), its relationship with data integration, and its safety properties.

%\subsection{An Illustrative Example}
%
%We first illustrate the algebra's main ideas using interaction examples in \Cref{f:teaser}.   A composition operator takes one or more views as operands and returns one or more views.  A user selects one or a set of ``source'' views, and drags them onto one or a set of ``destination'' (dest) views to specify a binary composition. For example, in \Cref{f:teaser}(a,b), the user drags the left chart onto the right chart, and then chooses the specific operator from a context menu,    The user can also select multiple views via a selection box or multi-clicking on views and apply an nary operator to the set of views.  In \Cref{f:teaser}(c,top), the user selects the CS and EE charts and executes a nary statistical composition operator that computes the averages between the departments. \Cref{f:teaser}(c,bottom) shows the user drag the average onto the set of CS and EE charts to subtract the average from each department's statistics.  In each example, the user chooses the specific comparison operator explicitly from a menu.   When the user selects a source view to initiate a composition interaction, charts that would result in unsafe compositions are disabled.
%

\subsection{Overview}\label{ss:vcaoverview}

This subsection presents the main operators in \sys, and how a view (operand) is modeled.  Note that we do not consider layout-oriented composition (e.g., organizing views side by side) since it is well-studied~\cite{Chen2020CompositionAC} and already widely supported in practice.

\input{content/tables.tex}
\begin{figure}[th]
  \centering
  \vspace{-1em}
  \includegraphics[width=.4\columnwidth]{viewtypes}
  \vspace{-1em}
  \caption{Bar chart of left-most table in \Cref{t:viewtypes}.  Its views include  the chart, a constant value, mark(s), and grouping attribute(s). }
  \label{f:viewtypes}
\end{figure}


\stitle{Operands:} 
A {\it view} traditionally refers to an entire chart.  In contrast, \sys defines view as the output of $R(T)$, where $T$ is a table (a raw table or a SQL query result) and $R$ is a visual encoding specification from a subset of $T$'s data attributes to visual attributes.  For example, \Cref{f:viewtypes} illustrates a bar chart that renders table \circled{1} in \Cref{t:viewtypes}, where $R$ is encodes \texttt{Date} to the x-axis, \texttt{src} to color, and the measure \texttt{Delay} to the y-axis.   We call $T$'s attributes its {\it schema}.   Similar to VizQL~\cite{Stolte2000PolarisAS}, the attributes in $T$ are either dimensions (used for filtering, grouping, and database joins) or measures (used to compute statistics); for ease of discussion, we will assume that each table contains a single measure.    The data rows in $T$ are mapped 1-to-1 into rendered marks in the view, and any computations and transformations necessary have already been applied to produce $T$ (in other words, $T$ is the output of a query).   Any part of the visualization that conforms to this definition as a {\it view}.   


We use \Cref{f:viewtypes} and \Cref{t:viewtypes} to illustrate the above concepts.  The chart is annotated with the different types of views that can be expressed as the tables listed in \Cref{t:viewtypes}.  
For instance, the chart's input table is depicted as \circled{1}. A constant value is a single-row table with a single attribute (\circled{2}), and a mark is a row from the input table (\circled{3}). A grouping attribute rendered in the legend represents a subset of rows that match a predicate: \texttt{SFO} corresponds to the rows that match \texttt{src=SFO} (\circled{4}).  Finally, predictive models use a subset of the dimension attributes to predict a measure attribute.  For instance, \circled{5} uses \texttt{Date} and \texttt{src} to predict the expected \texttt{Delay}.  In essence, $T$ is an instance of a table sampled from the model.  


\stitle{Operators:} 
\sys defines unary, binary, and nary composition operators and two decomposition operators.  The binary operators {\it statistical composition} and {\it union composition} are respectively used to derive new statistics and superimpose/juxtapose the operands.  The nary operators generalize the binary operators to compute aggregate statistics and superimpose/juxtapose a set of views.  The unary {\it lift} operator transforms a view into a predictive model; this is useful when the views are technically safe to compose, but do not share the same attribute values.  For example, composing two views that render prices on even days and odd days is not meaningful  because each odd day does not have a counterpart to comparable against in the even days.   Lifting the even days view will interpolate its prices to odd days so that the composition produces a meaningful result.  Finally, the unary extract and explode operators are for view {\it decomposition}, where components of a view are extracted and turned into new standalone views.



\subsection{Composition as Data Integration}

Data integration~\cite{doan2012principles,batini1986comparative,Naumann2018SchemaM,batini1986comparative,christen2012data} is a research field that studies the problem of combining two (or more) tables into a single ``integrated'' table, and deals with two primary problems. {\it Schema matching} maps attributes in one schema to semantically equivalent attributes in the second schema.  For instance, which attributes in the schemas \texttt{(day, price)} and \texttt{(date, cost)} should match?    {\it Entity matching} maps  rows (i.e., entities) in one table to the ``comparable'' rows (i.e., the same entities) in the second table.  

The same two problems manifest in view composition.  Determining whether the views are composable is an instance of schema matching.  For instance, a chart of \texttt{profits} vs \texttt{losses} should clearly not be composed with a chart of \texttt{names} vs \texttt{age}. However, it would also be ambiguous to compose with a chart of \texttt{profits} vs \texttt{profits} (of different years) since it is unclear which \texttt{profits} attribute in the latter chart should be matched with \texttt{profits} in the first chart.  

Similarly, determining which marks in the input views should be compared is an instance of entity matching because each mark renders a single input row.    For example, suppose we wish to compose the chart in \Cref{f:viewtypes}, whose dates span $1-3$, with a different chart whose dates span $5-8$.  Although their schemas are identical, none of the marks in the first view can be compared with any marks in the second view because their dates do not overlap.

 In short, the schema matching problem determines whether or not composition should be allowed (safety), whereas the entity matching helps us asses whether the composed view return a meaningful result.  In SQL terminology, the former determines if a join is possible, and the latter determines if the join would return any results.    This correspondence informs our definition and data-oriented approach to safety.

\subsection{Safety and Expressiveness}
\label{ss:criteria}

When is the data from multiple views safe to compose?
Determining the answer is necessary before defining {\it how} the views can be composed.
We now define an algebra's safety and expressiveness properties, and the heuristic rules that \sys uses.



\subsubsection{Safety}
Safety is needed to avoid compositions that are ambiguous, or may mislead the user.  For instance, a chart of \texttt{delay} by \texttt{date} should not be composed with a chart of \texttt{profits} by \texttt{market}.   \sys enforces safety by only allowing compositions for which there is a unique schema matching between the views' schemas.  To do so, \sys uses the following heuristic: two views are incompatible if their schemas cannot be unambiguously matched or if their measures are incompatible.  

Two tables match if their set of dimension attributes are the same and there are no duplicate attributes to cause ambiguity.  For binary operators, the dimensions may also have a superset-subset relationship (\Cref{s:algebra}).  Using this heuristic, the views in the above example do not match because their dimensions (\texttt{date}, \texttt{market}) do not overlap.   

Two measure attributes are compatible if they are derived from the same input attribute and use compatible statistical functions (if any) as determined by our attribute-sensitive type checking rules.  A function $f(a)$ can have output type $a$, a custom type $T$, or a parameterized custom type ${T}{<}{a}{>}$.  For instance, \texttt{average(a)}, \texttt{std(a)}, \texttt{min(a)}, and \texttt{max(a)} all output the type $a$, whereas \texttt{count(a)} outputs type $count{<}{a}{>}$.  Function evaluations are compatible if their output types are the same.  For instance, \texttt{avg(delay)} is compatible with \texttt{delay} and \texttt{min(delay)}, but not with \texttt{avg(price)} nor \texttt{count(delay)}.  


\subsubsection{Expressiveness} 
Expressiveness states that views that {\it could} be composed are allowed by the algebra.   For instance, a bar chart of September \texttt{profits} by \texttt{date} should be composable with a scatterplot of October \texttt{profits} by \texttt{date}.  To achieve this, \sys uses the view's table schema rather than its visual mapping to determine view compatibility. 
% 
Of course, there are many compositions that appear sensible to the user, but are disallowed based on our safety heuristics.   For instance, it is natural to compare a chart of \texttt{profits} with a chart of \texttt{losses} because (based on domain knowledege), we know that profits and losses are compatible.   To address this issue, we issue a warning when the user expresses an unsafe composition, and allow the user to override it in a special case: if the dimension attributes match, and the measure attributes are both numeric.
\Cref{s:discussion} discusses additional ways to expand expressiveness.




==> content/system.tex <==
\section{Implementation}

Implemented in ES6, renders charts using vega-lite, generates SQL queries executed in a database (currently SQLite or Google BigQuery). 

\subsection{Rendering}
Simple rules.


==> content/tables.tex <==
\begin{table}
  \small
  \begin{minipage}[t]{.34\linewidth}
    \centering
    \parbox[t]{\linewidth}{
      \begin{tabular}{ccr}
        \multicolumn{3}{c}{\circled{1} \textbf{Chart}}\\
        Date&Src&\blue{Delay}\\
        \hline
        1&SFO&\blue{10}\\
        2&SFO&\blue{15}\\
        3&SFO&\blue{20}\\
        1&OAK&\blue{15}\\
        2&OAK&\blue{10}\\
        3&OAK&\blue{5}\\
      \end{tabular}
    }
  \end{minipage}
  \hfill
  \begin{minipage}{.63\linewidth}
    \begin{minipage}[t]{\linewidth}
    \centering
    \parbox[t]{.3\textwidth}{
      \begin{tabular}{c}
        \multicolumn{1}{c}{\circled{2} \textbf{Value}}\\
        \blue{Delay}\\\hline
        \blue{20}
      \end{tabular}
    }
    \hfill
    \parbox[t]{.68\textwidth}{
      \begin{tabular}{ccr}
        \multicolumn{3}{c}{\circled{3} \textbf{Mark(s)}}\\
        Date&Src&\blue{Delay}\\
        \hline
        1&SFO&\blue{10}
      \end{tabular}
    }
    \end{minipage}
    \begin{minipage}{\linewidth}
      \parbox[t]{.52\textwidth}{
        \begin{tabular}{ccr}
          \multicolumn{3}{c}{\circled{4} \textbf{Group (b=2)}}\\
          Date&Src&\blue{Delay}\\
          \hline
          1&OAK&\blue{15}\\
          2&OAK&\blue{10}\\
          3&OAK&\blue{5}
        \end{tabular}
      }
      \hfill
      \parbox[t]{.42\textwidth}{
        \begin{tabular}{ccc}
          \multicolumn{3}{c}{\circled{5} \textbf{Model}}\\
          \multicolumn{3}{c}{$f(Date,Src)\to \blue{Delay}$}\\
          &&\\
          &&
        \end{tabular}
      }
    \end{minipage}
  \end{minipage}
  \vspace{1em}
  \caption{Tabular representation of charts, constant values, marks, groups, and predictive models.
  Dimensions in black, measures in \blue{blue}}
  \label{t:viewtypes}
\end{table}

